Capacity, Technology Portfolios, and the Paradox of Concentration

Does limiting the largest firm's capacity always lower prices? We model firms competing in supply schedules with multiple technologies, each with constant marginal cost up to capacity. In a tractable model, in which capacity and technological efficiency coexist as distinct sources of market power, we find that when the largest firm leads by efficiency, a small transfer of higher-cost capacity to the leader raises concentration yet lowers prices, contrary to standard antitrust intuition. Larger transfers raise prices, restoring standard intuition and tracing a non-monotone price-concentration relation. We prove existence and uniqueness of equilibrium, derive closed-form conditions for when transfers raise or lower prices, and extend the results to other oligopoly models. Evidence from Colombia's wholesale electricity market, where weather shocks shift hydropower capacity across technology-diversified firms, supports the pattern. Counterfactual transfers lower prices up to 30% in the least concentrated markets. We draw implications for capacity caps, divestitures, and mergers.

==> Figures/Model_fit/Regressions_Fit.tex <==

\begin{table}[htbp]
   \caption{Goodness of Fit: Simulated vs Real Data}
   \centering
   \begin{tabular}{lccc}
      \tabularnewline \midrule \midrule
      Dependent Variables:    & log(p)         & log(q)         & log(dat\_water)\\   
      Model:                  & (1)            & (2)            & (3)\\  
      \midrule
      \emph{Variables}\\
      Simulated Prices (ln)   & 0.9948$^{***}$ &                &   \\   
                              & (0.0006)       &                &   \\   
      Simulated Quantity (ln) &                & 0.9892$^{***}$ &   \\   
                              &                & (0.0033)       &   \\   
      Simulated Water (ln)    &                &                & 0.9823$^{***}$\\   
                              &                &                & (0.0017)\\   
      \midrule
      \emph{Fit statistics}\\
      Observations            & 29,943         & 26,672         & 1,103\\  
      R$^2$                   & -1.1677        & -4.6307        & -0.19314\\  
      Adjusted R$^2$          & -1.1677        & -4.6307        & -0.19314\\  
      \midrule \midrule
      \multicolumn{4}{l}{\emph{Heteroskedasticity-robust standard-errors in parentheses}}\\
      \multicolumn{4}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\
   \end{tabular}
\end{table}




==> Figures/Model_fit/Regressions_Water_Fit.tex <==

\begin{table}[htbp]
   \caption{Water Usage: Simulated vs Data}
   \centering
   \begin{tabular}{lcc}
      \tabularnewline \midrule \midrule
      Dependent Variables: & log(sim\_water)  & sim\_water\\   
                           & log(sim water)   & sim water \\   
      Model:               & (1)              & (2)\\  
      \midrule
      \emph{Variables}\\
      Constant             & 2.921$^{***}$    & 12,392.1$^{***}$\\   
                           & (0.3672)         & (850.0)\\   
      log(data water)      & 0.7260$^{***}$   &   \\   
                           & (0.0352)         &   \\   
      data water           &                  & 0.8084$^{***}$\\   
                           &                  & (0.0256)\\   
      \midrule
      \emph{Fit statistics}\\
      Observations         & 1,103            & 1,103\\  
      R$^2$                & 0.31483          & 0.31796\\  
      Adjusted R$^2$       & 0.31421          & 0.31734\\  
      \midrule \midrule
      \multicolumn{3}{l}{\emph{Clustered (nweek) standard-errors in parentheses}}\\
      \multicolumn{3}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\
   \end{tabular}
\end{table}




==> Figures/Model_fit/Table_Hourly_Diff_Pooled.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Wed, Feb 18, 2026 - 08:58:25 AM
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}} ccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Hour & RMSE (\%) & Hour.1 & RMSE (\%).1 & Hour.2 & RMSE (\%).2 & Hour.3 & RMSE (\%).3 & Hour.4 & RMSE (\%).4 \\ 
\hline \\[-1.8ex] 
1 & 0 & $75.25$ & 5 & $71.91$ & 10 & $45.45$ & 15 & $45.89$ & 20 & $39.49$ \\ 
2 & 1 & $79.14$ & 6 & $68.85$ & 11 & $43.61$ & 16 & $46.09$ & 21 & $43.18$ \\ 
3 & 2 & $82.21$ & 7 & $60.27$ & 12 & $44.46$ & 17 & $46.42$ & 22 & $53.16$ \\ 
4 & 3 & $83.17$ & 8 & $53.15$ & 13 & $45.60$ & 18 & $38.70$ & 23 & $67.42$ \\ 
5 & 4 & $80.25$ & 9 & $49.80$ & 14 & $45.05$ & 19 & $38.03$ & All & $55.76$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> Figures/Model_fit/Table_Water_Fit_ByFirm.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Wed, Feb 18, 2026 - 09:12:26 AM
\begin{table}[!htbp] \centering 
  \caption{Water Usage Fit: Simulated vs Data (by Firm)} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}} ccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Focal\_Agent & N & Corr & RMSE & Mean\_Error & Mean\_Abs\_Error \\ 
\hline \\[-1.8ex] 
1 & ENDG & $312$ & $0.145$ & $20,135.520$ & $6,912.021$ & $17,620.920$ \\ 
2 & EPMG & $312$ & $0.257$ & $15,389.870$ & $7,629.425$ & $12,618.870$ \\ 
3 & EPSG & $312$ & $0.142$ & $8,517.923$ & $457.650$ & $7,237.719$ \\ 
4 & ISGG & $312$ & $0.031$ & $19,483.670$ & $3,261.743$ & $16,215.400$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> Tables/structural_model/res2_p4_c1.tex <==
\begin{table}[ht]\caption{Estimated primitives -- four spline parameters \label{tab:estimates_p4} }
\begin{center}
\begin{adjustbox}{width=.9\textwidth,center}
\begin{tabular}{l*{4}{r @{} l}}
\toprule
                 &         (1)&        &         (2)&        &         (3)&        &         (4)&        \\
\midrule
\multicolumn{9}{c}{\textbf{Marginal costs (COP/MWh)}} \\
Thermal $(\psi^{thermal})$&    194897.17&$^{***}$&    157783.19&$^{***}$&    194739.39&$^{***}$&    149699.10&$^{***}$\\
                &  (23,815.33)&        &  (30,285.54)&        &  (23,816.43)&        &  (31,060.26)&        \\
Hydropower $(\psi^{hydro})$&    117918.58&$^{***}$&    68,920.91&        &    127323.61&$^{***}$&    51,297.15&        \\
                &  (15,763.87)&        &  (109793.29)&        &  (15,236.51)&        &  (66,230.75)&        \\
\multicolumn{9}{c}{\textbf{Intertemporal value of water (COP/MWh)}} \\                
Spline 1 $(\gamma_1)$&   --4,172.94&        &     3,466.69&        &       555.13&        &    10,797.46&        \\
                &   (5,199.93)&        &   (4,433.25)&        &   (2,860.60)&        &   (6,706.77)&        \\
Spline 2 $(\gamma_2)$&  --1.914e-03&        &  --2.502e-03&        &  --2.985e-03&$^{*}$  &  --3.576e-03&$^{*}$  \\
                &  (1.431e-03)&        &  (2.011e-03)&        &  (1.493e-03)&        &  (1.961e-03)&        \\
Spline 3 $(\gamma_3)$&    6.524e-09&$^{*}$  &    1.599e-08&$^{*}$  &    9.504e-09&$^{*}$  &    1.382e-08&$^{*}$  \\
                &  (3.325e-09)&        &  (8.588e-09)&        &  (4.730e-09)&        &  (7.090e-09)&        \\
Spline 4 $(\gamma_4)$&    1.470e-08&        &  --2.310e-08&        &  --4.796e-09&        &  --1.996e-08&        \\
                &  (9.490e-09)&        &  (2.091e-08)&        &  (9.418e-09)&        &  (1.420e-08)&        \\
\multicolumn{9}{c}{\textbf{Fixed Effects}} \\
Firm        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        \\
Generator   &             &        &             &        &             &        & $\checkmark$&        \\
Month-by-technology&             &        & $\checkmark$&        &             &        & $\checkmark$&        \\
Hour        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        \\
Week-by-year& $\checkmark$&        & $\checkmark$&        &             &        &             &        \\
Date        &             &        &             &        & $\checkmark$&        & $\checkmark$&        \\
\midrule
Clustered s.e.  &    Generator&        &    Generator&        &    Generator&        &    Generator&        \\
SW F $(\psi^{thermal})$&        32.93&        &       842.34&        &        30.56&        &       129.27&        \\
SW F $(\psi^{hydro})$&       147.35&        &       192.14&        &       130.37&        &     1,628.33&        \\
SW F $(\gamma_1)$&       469.69&        &       869.78&        &       568.03&        &       249.90&        \\
SW F $(\gamma_2)$&       664.20&        &       415.03&        &       233.01&        &       370.99&        \\
SW F $(\gamma_3)$&        65.98&        &        80.57&        &       537.50&        &       172.45&        \\
SW F $(\gamma_4)$&        26.91&        &        15.47&        &       752.78&        &        55.22&        \\
Anderson Rubin F&        19.74&        &        43.46&        &       196.42&        &       106.90&        \\
KP Wald         &         5.74&        &         9.41&        &         8.47&        &        21.39&        \\
Overid. p-value &         0.15&        &         0.13&        &         0.10&        &         0.16&        \\
N               &    1,451,592&        &    1,451,592&        &    1,451,592&        &    1,451,592&        \\
\bottomrule
\multicolumn{9}{l}{* -- $p < 0.1$; ** -- $p < 0.05$; *** -- $p < 0.01$}
\end{tabular}
\end{adjustbox}
\end{center}
\begin{tablenotes}\footnotesize
\item Notes: This table presents the coefficients obtained estimating (\ref{eq:2sls}) by two-stage least squares on daily data between January 1, 2010, and December 31, 2015. Unlike the results presented in the main text (Table \ref{tab:estimates}), these estimates are based on an approximation of the value function over four knots instead of five, meaning that we estimate only four $\{\gamma\}_{r=1}^4$. The top panels separate the marginal cost estimates and the value function parameters from the fixed effects used in estimation, which vary across columns. Our favorite specification is in Column (4), which includes day-fixed effects. The bottom panel provides diagnostic tests in the first stage. The standard errors are clustered at the level of the generator. 2,900 COP $\simeq$ 1 US\$
\end{tablenotes}
\end{table}


==> Tables/structural_model/res2_p4_c1_normal.tex <==
\begin{table}[ht]\caption{Estimated primitives -- employing a normal density for the transition matrix \label{tab:estimates_p4_normal} }
\begin{center}
\begin{adjustbox}{width=.9\textwidth,center}
\begin{tabular}{l*{4}{r @{} l}}
\toprule
                 &         (1)&        &         (2)&        &         (3)&        &         (4)&        \\
\midrule
\multicolumn{9}{c}{\textbf{Marginal costs (COP/MWh)}} \\
Thermal $(\psi^{thermal})$&    195,271.35&$^{***}$&    152,621.02&$^{***}$&    194,831.41&$^{***}$&    151,112.79&$^{***}$\\
                &  (23,993.80)&        &  (30,884.62)&        &  (23,621.62)&        &  (30,492.26)&        \\
Hydropower $(\psi^{hydro})$&    120408.48&$^{***}$&    32,919.28&        &    128840.47&$^{***}$&    59,085.78&        \\
                &  (16,258.70)&        &  (78,427.99)&        &  (15,439.79)&        &  (63,782.79)&        \\
\multicolumn{9}{c}{\textbf{Intertemporal value of water (COP/MWh)}} \\
Spline 1 $(\gamma_1)$&   --2,720.98&        &     6,297.20&        &     1,569.04&        &    10,291.14&        \\
                &   (5,204.24)&        &   (5,100.84)&        &   (3,059.75)&        &   (6,504.18)&        \\
Spline 2 $(\gamma_2)$&  --2.752e-03&$^{*}$  &  --2.829e-03&        &  --3.485e-03&$^{**}$ &  --3.836e-03&$^{*}$  \\
                &  (1.534e-03)&        &  (2.031e-03)&        &  (1.649e-03)&        &  (2.136e-03)&        \\
Spline 3 $(\gamma_3)$&    7.278e-09&$^{*}$  &    1.527e-08&$^{*}$  &    1.025e-08&$^{*}$  &    1.538e-08&$^{*}$  \\
                &  (3.639e-09)&        &  (8.119e-09)&        &  (5.077e-09)&        &  (7.788e-09)&        \\
Spline 4 $(\gamma_4)$&    1.844e-08&        &  --2.010e-08&        &  --4.491e-09&        &  --2.165e-08&        \\
                &  (1.183e-08)&        &  (1.624e-08)&        &  (1.016e-08)&        &  (1.494e-08)&        \\
\multicolumn{9}{c}{\textbf{Fixed Effects}} \\
FE: Firm        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        \\
FE: Generator   &             &        & $\checkmark$&        &             &        & $\checkmark$&        \\
FE: Month-by-technology&             &        & $\checkmark$&        &             &        & $\checkmark$&        \\
FE: Hour        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        \\
FE: Week-by-year& $\checkmark$&        & $\checkmark$&        &             &        &             &        \\
FE: Date        &             &        &             &        & $\checkmark$&        & $\checkmark$&        \\
\midrule
% Clustered s.e.  &    Generator&        &    Generator&        &    Generator&        &    Generator&        \\
SW F $(\psi^{thermal})$&     3,248.74&        &       802.28&        &     2,900.21&        &       750.10&        \\
SW F $(\psi^{hydro})$&     1,561.65&        &       253.23&        &     1,934.29&        &       344.08&        \\
SW F $(\gamma_1)$&       433.52&        &       249.50&        &       533.06&        &       277.42&        \\
SW F $(\gamma_2)$&       465.61&        &       281.87&        &       488.30&        &       330.92&        \\
SW F $(\gamma_3)$&       663.30&        &       477.94&        &       750.50&        &       491.06&        \\
SW F $(\gamma_4)$&       740.30&        &       440.92&        &       734.06&        &       446.90&        \\
Anderson Rubin F&     2,055.72&        &     1,395.05&        &     2,437.39&        &     1,539.08&        \\
KP Wald         &       139.94&        &       182.54&        &       239.48&        &       183.28&        \\
Overid. p-value &         0.00&        &         0.00&        &         0.00&        &         0.00&        \\
N               &    1,451,592&        &    1,451,592&        &    1,451,592&        &    1,451,592&        \\
\bottomrule
\multicolumn{9}{l}{* -- $p < 0.1$; ** -- $p < 0.05$; *** -- $p < 0.01$}
\end{tabular}
\end{adjustbox}
\end{center}
\begin{tablenotes}\footnotesize
\item Notes: This table presents the coefficients obtained estimating (\ref{eq:2sls}) by two-stage least squares on daily data between January 1, 2010, and December 31, 2015. Unlike the results presented in the main text (Table \ref{tab:estimates}), these estimates assume that the transition matrix is normally distributed and are based on an approximation of the value function over four knots instead of five, meaning that we estimate only four $\{\gamma\}_{r=1}^4$. The top panels separate the marginal cost estimates and the value function parameters from the fixed effects used in estimation, which vary across columns. Our favorite specification is in Column (4), which includes day-fixed effects. The bottom panel provides diagnostic tests in the first stage. 2,900 COP $\simeq$ 1 US\$
\end{tablenotes}
\end{table}


==> Tables/structural_model/res2_p4_rob_normal.tex <==
\begin{table}[!ht]\caption{Estimated model primitives---employing a normal density for the transition matrix  and 4 polynomials for $V(\cdot)$\label{tab:estimates_p4_normal} }
\begin{center}
\begin{adjustbox}{width=.9\textwidth,center}
\begin{tabular}{l*{4}{r @{} l}}
\toprule
                 &         (1)&        &         (2)&        &         (3)&        &         (4)&        \\
\midrule
\multicolumn{9}{c}{\textbf{Marginal costs (COP/MWh)}} \\
Thermal $(c^{T})$&    195271.35&$^{***}$&    152621.02&$^{***}$&    194831.41&$^{***}$&    151112.79&$^{***}$\\
                &   (1,605.71)&        &   (1,807.59)&        &   (1,229.58)&        &   (1,573.39)&        \\
Hydropower $(c^{H})$&    120408.48&$^{***}$&    32,919.28&$^{***}$&    128840.47&$^{***}$&    59,085.78&$^{***}$\\
                &   (1,313.47)&        &   (5,997.03)&        &     (871.55)&        &   (4,459.66)&        \\
\multicolumn{9}{c}{\textbf{Intertemporal value of water (COP/MWh)}} \\
Spline 1 $(\gamma_1)$&   --2,720.98&$^{***}$&     6,297.20&$^{***}$&     1,569.04&$^{***}$&    10,291.14&$^{***}$\\
                &     (635.73)&        &     (515.56)&        &     (329.00)&        &     (461.14)&        \\
Spline 2 $(\gamma_2)$&  --2.752e-03&$^{***}$&  --2.829e-03&$^{***}$&  --3.485e-03&$^{***}$&  --3.836e-03&$^{***}$\\
                &  (2.242e-04)&        &  (1.588e-04)&        &  (1.235e-04)&        &  (1.425e-04)&        \\
Spline 3 $(\gamma_3)$&    7.278e-09&$^{***}$&    1.527e-08&$^{***}$&    1.025e-08&$^{***}$&    1.538e-08&$^{***}$\\
                &  (7.491e-10)&        &  (6.213e-10)&        &  (4.369e-10)&        &  (5.414e-10)&        \\
Spline 4 $(\gamma_4)$&    1.844e-08&$^{***}$&  --2.010e-08&$^{***}$&  --4.491e-09&$^{***}$&  --2.165e-08&$^{***}$\\
                &  (2.351e-09)&        &  (1.804e-09)&        &  (1.222e-09)&        &  (1.550e-09)&        \\
\multicolumn{9}{c}{\textbf{Fixed Effects}} \\
FE: Firm        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        \\
FE: Unit   &             &        & $\checkmark$&        &             &        & $\checkmark$&        \\
FE: Month-by-technology&             &        & $\checkmark$&        &             &        & $\checkmark$&        \\
FE: Hour        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        \\
FE: Week-by-year& $\checkmark$&        & $\checkmark$&        &             &        &             &        \\
FE: Date        &             &        &             &        & $\checkmark$&        & $\checkmark$&        \\
\midrule
SW F $(c^{Y})$&        36.41&        &       113.62&        &        34.13&        &        94.59&        \\
SW F $(c^{H})$&       124.43&        &       300.57&        &       139.18&        &     2,474.37&        \\
SW F $({\gamma_1})$&       616.23&        &       652.90&        &       483.22&        &       617.59&        \\
SW F $({\gamma_2})$&     1,401.71&        &       364.00&        &       194.38&        &       284.03&        \\
SW F $({\gamma_3})$&        76.56&        &        93.11&        &       644.24&        &       248.55&        \\
SW F $({\gamma_4})$&        45.66&        &        86.99&        &     1,139.58&        &        82.71&        \\
Anderson Rubin F&        19.74&        &       111.61&        &       196.42&        &       106.90&        \\
KP Wald         &         7.16&        &        10.80&        &         6.61&        &        19.28&        \\
% Overid. p-value &         0.19&        &         0.21&        &         0.11&        &         0.14&        \\
N               &    1,451,592&        &    1,451,592&        &    1,451,592&        &    1,451,592&        \\
\bottomrule
\multicolumn{9}{l}{* -- $p < 0.1$; ** -- $p < 0.05$; *** -- $p < 0.01$}
\end{tabular}
\end{adjustbox}
\end{center}
\begin{tablenotes}\footnotesize
\item Notes: This table presents the coefficients obtained estimating (\ref{eq:2sls}) by two-stage least squares on daily data between January 1, 2010, and December 31, 2015. Unlike the results presented in the main text (Table \ref{tab:estimates}), these estimates assume that the transition matrix is normally distributed and are based on an approximation of the value function over four knots instead of five, meaning that we estimate only four $\{\gamma\}_{r=1}^4$. The top panels separate the marginal cost estimates and the value function parameters from the fixed effects used in estimation, which vary across columns. Our favorite specification is in Column (4), which includes day-fixed effects. The bottom panel provides diagnostic tests in the first stage. 2,900 COP $\simeq$ 1 US\$
\end{tablenotes}
\end{table}


==> Tables/structural_model/res2_p5_c1.tex <==
\begin{table}[ht!]\caption{Estimated model primitives \label{tab:estimates}}
\centering
\begin{adjustbox}{width=.9\textwidth,center}
\begin{tabular}{l*{4}{r @{} l}}
\toprule
                &         (1)&        &         (2)&        &         (3)&        &         (4)&        \\
\midrule
\multicolumn{9}{c}{\textbf{Marginal Costs (COP/MWh)}} \\
Thermal $(\psi^{thermal})$&    203,677.62&$^{***}$&    141,668.46&$^{***}$&    221,304.18&$^{***}$&    144,744.21&$^{***}$\\
                &  (27,089.82)&        &  (25,973.12)&        &  (30,676.82)&        &  (24,760.50)&        \\
Hydropower $(\psi^{hydro})$&    64,258.02&        &    20,123.07&        &    29,187.79&        &    52,755.37&        \\
                &  (47,367.32)&        &  (73,680.43)&        &  (37,949.09)&        &  (54,774.84)&        \\
\multicolumn{9}{c}{\textbf{Intertemporal Value of Water (COP/MWh)}} \\
Spline 1 $(\gamma_1)$&   --2,950.20&        &   --6,812.77&        &   --11,664.64&$^{*}$  &   --3,812.18&        \\
                &   (3,871.73)&        &   (5,343.19)&        &   (6,316.13)&        &   (4,432.24)&        \\
Spline 2 $(\gamma_2)$&  --2.301e-03&        &  --1.546e-04&        &    6.286e-04&        &  --8.402e-04&        \\
                &  (1.417e-03)&        &  (1.550e-03)&        &  (2.151e-03)&        &  (1.436e-03)&        \\
Spline 3 $(\gamma_3)$&  --3.527e-09&        &    1.919e-08&$^{*}$  &  --1.932e-08&        &    1.712e-08&$^{*}$  \\
                &  (6.771e-09)&        &  (1.049e-08)&        &  (1.835e-08)&        &  (9.323e-09)&        \\
Spline 4 $(\gamma_4)$&    3.246e-08&$^{*}$  &  --3.119e-08&$^{*}$  &    4.536e-08&        &  --2.729e-08&$^{*}$  \\
                &  (1.897e-08)&        &  (1.667e-08)&        &  (3.544e-08)&        &  (1.487e-08)&        \\
Spline 5 $(\gamma_5)$&  --1.414e-08&        &    9.357e-08&$^{**}$ &    5.167e-08&$^{**}$ &    8.566e-08&$^{**}$ \\
                &  (2.569e-08)&        &  (4.023e-08)&        &  (2.446e-08)&        &  (3.565e-08)&        \\
\multicolumn{9}{c}{\textbf{Fixed Effects}} \\
Firm        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        \\
Generator   & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        \\
Month-by-technology&             &        & $\checkmark$&        &             &        & $\checkmark$&        \\
Hour        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        \\
Week-by-year& $\checkmark$&        & $\checkmark$&        &             &        &             &        \\
Date        &             &        &             &        & $\checkmark$&        & $\checkmark$&        \\
\midrule
Clustered s.e.  &    Generator&        &    Generator&        &    Generator&        &    Generator&        \\
SW F $(\psi^{thermal})$&       194.34&        &       162.86&        &     1,919.25&        &       168.62&        \\
SW F $(\psi^{hydro})$&       497.69&        &       422.00&        &       634.45&        &     1,321.92&        \\
SW F $({\gamma_1})$&       540.51&        &     1,469.70&        &       291.62&        &       157.63&        \\
SW F $({\gamma_2})$&       496.05&        &     1,332.65&        &       459.68&        &       143.17&        \\
SW F $({\gamma_3})$&       218.39&        &       121.81&        &     1,070.14&        &       162.82&        \\
SW F $({\gamma_4})$&        73.20&        &        63.96&        &       804.80&        &        51.49&        \\
SW F $({\gamma_5})$&       160.13&        &       159.37&        &       291.35&        &       102.47&        \\
Anderson Rubin F&        10.30&        &       111.61&        &        70.19&        &       106.90&        \\
KP Wald         &        20.62&        &        16.49&        &        12.08&        &        35.80&        \\
Overid. p-value &         0.14&        &         0.29&        &         0.25&        &         0.23&        \\
N               &    1,451,592&        &    1,451,592&        &    1,451,592&        &    1,451,592&        \\
\bottomrule
\multicolumn{9}{l}{* -- $p < 0.1$; ** -- $p < 0.05$; *** -- $p < 0.01$}
\end{tabular}%
\end{adjustbox}
\begin{tablenotes} \footnotesize
\item Notes: This table presents the coefficients obtained estimating (\ref{eq:2sls}) by two-stage least squares on daily data between January 1, 2010, and December 31, 2015. The top panels separate the marginal cost estimates and the value function parameters from the fixed effects used in estimation, which vary across columns. Our favorite specification is in Column (4), which includes day-fixed effects. The bottom panel provides diagnostic tests in the first stage. The standard errors are clustered at the level of the generator. 2,900 COP $\simeq$ 1 US\$.
\end{tablenotes}
\end{table}


==> Tables/structural_model/res2_p5_c1_normal.tex <==
\begin{table}[ht]\caption{Estimated primitives -- employing a normal density for the transition matrix \label{tab:estimates_normal} }
\begin{center}
\begin{adjustbox}{width=.9\textwidth,center}
\begin{tabular}{l*{4}{r @{} l}}
\toprule
                 &         (1)&        &         (2)&        &         (3)&        &         (4)&        \\
\midrule
\multicolumn{9}{c}{\textbf{Marginal costs (COP/MWh)}} \\
Thermal $(\psi^{thermal})$&    204,727.14&$^{***}$&    143,319.87&$^{***}$&    220,441.60&$^{***}$&    146,635.86&$^{***}$\\
                &  (28,325.54)&        &  (25,840.50)&        &  (30,818.24)&        &  (24,543.39)&        \\
Hydropower $(\psi^{hydro})$&    46,491.28&        &    28,163.59&        &    28,458.10&        &    60,353.00&        \\
                &  (52,823.03)&        &  (69,216.84)&        &  (37,397.66)&        &  (51,818.25)&        \\
\multicolumn{9}{c}{\textbf{Intertemporal value of water (COP/MWh)}} \\
Spline 1 $(\gamma_1)$&     --797.45&        &   --6,751.10&        &   --9,712.11&$^{*}$  &   --3,744.90&        \\
                &   (3,944.05)&        &   (5,278.98)&        &   (5,659.04)&        &   (4,094.15)&        \\
Spline 2 $(\gamma_2)$&  --3.346e-03&$^{*}$  &  --3.154e-04&        &  --2.173e-04&        &  --1.064e-03&        \\
                &  (1.695e-03)&        &  (1.657e-03)&        &  (2.093e-03)&        &  (1.500e-03)&        \\
Spline 3 $(\gamma_3)$&  --4.894e-09&        &    2.009e-08&$^{*}$  &  --1.621e-08&        &    1.837e-08&$^{*}$  \\
                &  (8.692e-09)&        &  (1.091e-08)&        &  (1.744e-08)&        &  (9.650e-09)&        \\
Spline 4 $(\gamma_4)$&    4.070e-08&        &  --3.179e-08&$^{*}$  &    4.205e-08&        &  --2.848e-08&$^{*}$  \\
                &  (2.422e-08)&        &  (1.698e-08)&        &  (3.381e-08)&        &  (1.501e-08)&        \\
Spline 5 $(\gamma_5)$&  --2.216e-08&        &    8.949e-08&$^{**}$ &    4.422e-08&$^{*}$  &    8.251e-08&$^{**}$ \\
                &  (2.844e-08)&        &  (3.901e-08)&        &  (2.212e-08)&        &  (3.421e-08)&        \\
\multicolumn{9}{c}{\textbf{Fixed Effects}} \\ Firm        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        \\
Generator   & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        \\
Month-by-technology&             &        & $\checkmark$&        &             &        & $\checkmark$&        \\
Hour        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        & $\checkmark$&        \\
Week-by-year& $\checkmark$&        & $\checkmark$&        &             &        &             &        \\
FE: Date        &             &        &             &        & $\checkmark$&        & $\checkmark$&        \\               
\midrule
Clustered s.e.  &    Generator&        &    Generator&        &    Generator&        &    Generator&        \\
SW F $(\psi^{thermal})$&       154.12&        &       224.24&        &     1,529.34&        &       130.50&        \\
SW F $(\psi^{hydro})$&       516.90&        &       378.63&        &       715.46&        &     1,885.82&        \\
SW F $({\gamma_1})$&       995.28&        &     2,977.43&        &       344.76&        &       266.18&        \\
SW F $({\gamma_2})$&       125.25&        &     1,159.14&        &       533.56&        &       166.11&        \\
SW F $({\gamma_3})$&       310.90&        &       130.10&        &       423.58&        &       228.60&        \\
SW F $({\gamma_4})$&        83.29&        &        57.88&        &       998.67&        &        62.75&        \\
SW F $({\gamma_5})$&       181.17&        &        98.96&        &       298.75&        &       124.10&        \\
Anderson Rubin F&        10.30&        &       111.61&        &        70.19&        &       106.90&        \\
KP Wald         &        24.47&        &        13.34&        &        12.20&        &        26.58&        \\
Overid. p-value &         0.13&        &         0.29&        &         0.26&        &         0.22&        \\
N               &    1,451,592&        &    1,451,592&        &    1,451,592&        &    1,451,592&        \\
\bottomrule
\multicolumn{9}{l}{* -- $p < 0.1$; ** -- $p < 0.05$; *** -- $p < 0.01$}
\end{tabular}
\end{adjustbox}
\end{center}
\begin{tablenotes}\footnotesize
\item Notes: This table presents the coefficients obtained estimating (\ref{eq:2sls}) by two-stage least squares on daily data between January 1, 2010, and December 31, 2015. Unlike the results presented in the main text (Table \ref{tab:estimates}), these estimates assume that the transition matrix is normally distributed. The top panels separate the marginal cost estimates and the value function parameters from the fixed effects used in estimation, which vary across columns. Our favorite specification is in Column (4), which includes day-fixed effects. The bottom panel provides diagnostic tests in the first stage. The standard errors are clustered at the level of the generator. 2,900 COP $\simeq$ 1 US\$
\end{tablenotes}
\end{table}

